Omni2Web: Benchmarking Audiovisual Website Development

Screen-recorded web editing requests contain weak deictic expressions such as ``this'' and ``there,'' whose referents depend on speech, cursor trajectories, page state, and edit history. Such requests require intent recovery beyond the explicit specifications assumed by many existing web-editing benchmarks. We introduce Omni2Web, a bilingual benchmark of 918 instances spanning 13,907 edit steps. It defines three complementary tracks: Direct Editing evaluates webpage editing from recordings, Instruction Recovery measures explicit intent recovery, and Instruction Utility tests whether recovered instructions can drive a fixed code executor. We evaluate 17 open- and closed-source models. The best models attain 51.17 on the Edit Fidelity Score (EFS) for Direct Editing and 49.14 on the Instruction Recovery Score (IRS); under the fixed executor, the strongest recovered instructions reach 51.08 EFS, still far below the 89.69 EFS obtained with oracle instructions. Step-level analyses show that correct grounding does not guarantee successful edits, while some Omni models recover instructions that the fixed coding model executes substantially better than their direct edits. Controlled ablations further demonstrate the value of temporally aligned audiovisual evidence, while alternative judges preserve the leader and broad ordering. Together, these findings reveal substantial headroom in multimodal intent recovery and code execution and highlight the promise of pairing Omni rewriters with coding models.

==> title_brand.tex <==
\RequirePackage{accsupp}
\newsavebox{\omniinitialbox}

% Keep the title's text font and line height; replace only its initial O.
\DeclareRobustCommand{\omniwordmark}{%
  \texorpdfstring{%
    \begingroup
    \sbox{\omniinitialbox}{O}%
    \BeginAccSupp{method=escape,ActualText=Omni2Web}%
    \raisebox{-0.06em}[\ht\omniinitialbox][\dp\omniinitialbox]{%
      \includegraphics[height=0.95em]{figures/omni2web_o.pdf}%
    }%
    \kern-0.055em mni2Web%
    \EndAccSupp{}%
    \endgroup
  }{Omni2Web}%
}

